Angry Men, Sad Women: Large Language Models Reflect Gendered Stereotypes in Emotion Attribution

Large language models (LLMs) reflect societal norms and biases, especially about gender. While societal biases and stereotypes have been extensively researched in various NLP applications, there is a surprising gap for emotion analysis. However, emotion and gender are closely linked in societal discourse. E.g., women are often thought of as more empathetic, while men's anger is more socially accepted. To fill this gap, we present the first comprehensive study of gendered emotion attribution in five state-of-the-art LLMs (open- and closed-source). We investigate whether emotions are gendered, and whether these variations are based on societal stereotypes. We prompt the models to adopt a gendered persona and attribute emotions to an event like 'When I had a serious argument with a dear person'. We then analyze the emotions generated by the models in relation to the gender-event pairs. We find that all models consistently exhibit gendered emotions, influenced by gender stereotypes. These findings are in line with established research in psychology and gender studies. Our study sheds light on the complex societal interplay between language, gender, and emotion. The reproduction of emotion stereotypes in LLMs allows us to use those models to study the topic in detail, but raises questions about the predictive use of those same LLMs for emotion applications.

==> tables/dataset.tex <==
% \begin{table}[h]
%     \small
%     \centering
%     \begin{tabular}{lcc}
%     \toprule
%         \textbf{Emotion} & \textbf{Woman} & \textbf{Man} \\
%         \midrule
%         \anger  & 594 &  594\\
%         \disgust & 594 & 594 \\
%         \fear  & 597 & 597 \\
%         \sadness & 593 & 593\\
%         \joy & 597 & 597\\
%         \guilt & 590 & 590\\
%         \shame & 588 & 588 \\
%         \midrule
%         Total & 4,153 & 4,153 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Distribution of emotions per gender (female, male) in the ISEAR dataset.}
%     \label{tab:isear}
% \end{table}

==> tables/emotion_landscape.tex <==
\begin{table*}[t]
\small
\begin{tabularx}{\linewidth}{lX}
    \toprule
    \textbf{Emotion category} & \textbf{Emotion-related words}  \\
    \midrule
    \anger & frustration, betrayal, annoyance, irritation, resentment, exasperation, outrage, rage, humiliated, hate \\
    \disgust & revulsion, repulsion, nausea  \\
    \fear & anxiety, concern, panic, worry, apprehension, horror, vulnerability, jealousy, nervousness, defensiveness, terror \\
    \sadness & grief, disappointment, hurt, sorrow, pain, helplessness, resignation, loneliness, depression  \\
    \joy & excitement, serenity, ecstasy, relaxation, relief, surprise, pride, love, gratitude, satisfaction, happiness, amusement, empathy, contentment, euphoria, gladness %exhilaration  
    \\
    \guilt & regret, self-blame \\
    \shame & embarrassment, humiliation \\
    \bottomrule
\end{tabularx}
\caption{Some emotion-related words generated by the LMs per emotion category.}\label{tab:emotion_landscape}
\end{table*}

==> tables/frequencies.tex <==
\begin{table*}[!htp]
\centering
\begin{tabular}{l|rr|rr|rr|rr|rr|rr}\toprule
&\multicolumn{2}{c|}{Llama-7b} &\multicolumn{2}{c|}{Llama-13b} &\multicolumn{2}{c|}{Llama-70b} &\multicolumn{2}{c|}{Mistral-7b} &\multicolumn{2}{c}{GPT-4} \\\cmidrule{2-11}
    Emotion &Man &Woman &Man &Woman &Man &Woman &Man &Woman &Man &Woman \\\midrule
    Anger &0.413 &0.531 &0.660 &0.608 &0.666 &0.614 &0.591 &0.564 & & \\
    Disgust &0.406 &0.511 &0.707 &0.732 &0.627 &0.690 &0.611 &0.662 & & \\
    Fear &0.472 &0.622 &0.669 &0.782 &0.795 &0.856 &0.800 &0.830 & & \\
    Guilt &0.367 &0.474 &0.617 &0.568 &0.685 &0.724 &0.620 &0.657 & & \\
    Joy &0.898 &0.910 &0.926 &0.904 &0.925 &0.940 &0.947 &0.930 & & \\
    Sadness &0.639 &0.703 &0.862 &0.626 &0.744 &0.651 &0.635 &0.572 & & \\
    Shame &0.460 &0.537 &0.616 &0.655 &0.541 &0.595 &0.524 &0.604 & & \\
    \midrule
    Macro-avg &0.522 &0.612 &0.723 &0.696 &0.712 &0.724 &0.675 &0.688 & & \\
\bottomrule
\end{tabular}\caption{F1 scores of Mistral-7B, Llama2-(7B, 13B, 70B) and GPT-4 on the ISEAR dataset across emotions and gender (F: Female, M: Male). Persona Instruction: P2.}\label{tab:results} 
\end{table*}

==> x.tex <==

%Assigning specific emotions to genders can be problematic and perpetuate stereotypes. Emotions are complex and vary greatly among individuals, regardless of gender. Associating certain emotions with specific genders can contribute to harmful assumptions and reinforce gender norms. From a safety and ethical standpoint, it's generally better to treat emotions as universal experiences that can be expressed by anyone, regardless of their gender identity. Language models should aim to promote inclusivity, diversity, and avoid reinforcing stereotypes that might contribute to discrimination or bias. If a language model is designed to generate text or responses that involve emotions, it's important to ensure that the model is trained on diverse and inclusive datasets to reflect the wide range of human experiences. The goal should be to create models that are sensitive to the diversity of emotions and expressions across all genders.
%Traditional gender roles often prescribed specific ways in which men and women were expected to express their emotions. For example, anger might be more socially acceptable for men, while sadness or vulnerability might be more acceptable for women.
%In recent decades, there has been a gradual shift in societal expectations regarding gender and emotions. Efforts to challenge traditional stereotypes have sought to promote emotional expression and understanding for all gender


% Men as Rational, Women as Emotional:

% Historical Perspective: In many societies, especially in Western cultures, there has been a historical stereotype that men are more rational and logical, while women are more emotional and nurturing.
% Implications: This stereotype has often been used to justify gender roles, with men expected to take on leadership roles and women expected to focus on caregiving and emotional support.
% Suppression of Men's Emotions:

% Historical Perspective: Some societies have traditionally discouraged men from expressing vulnerability or emotions other than anger. Men were often expected to be stoic and not show signs of weakness.
% Implications: This stereotype could contribute to issues related to mental health, as men may feel pressure to suppress emotions that are considered "unmanly."
% Women as Hysterical:

% Historical Perspective: The term "hysteria" historically referred to a psychological disorder thought to affect women, characterized by emotional excess. This stereotype suggested that women were prone to irrational and unpredictable behavior due to their biology.
% Implications: The concept of hysteria has been largely discredited, but remnants of the stereotype may persist in the form of dismissing women's emotions as irrational.



%The perpetuation of gender biases in emotion analysis by language models can be harmful on various levels. Firstly, it reinforces and amplifies existing societal stereotypes and norms, contributing to the marginalization and misrepresentation of certain gender groups. This not only perpetuates gender inequality but also limits the scope of understanding and expressing emotions within diverse gender experiences.

% In applications like writing referenced letters, these biases can have direct and tangible consequences. For instance, if a language model consistently associates females with emotions like sadness and empathy and males with anger and pride, it may inadvertently inject biased language into reference letters. This can result in unintentional reinforcement of gender stereotypes, potentially influencing how individuals are perceived and evaluated in professional or academic contexts. Such biases may contribute to the perpetuation of gender-based disparities and hinder efforts towards creating fair and inclusive environments.

% Addressing these issues involves refining language models to be more conscious of and responsive to diverse gender expressions, ensuring that applications like writing reference letters are free from gender-based biases and contribute to a more equitable and inclusive representation of individuals. This includes ongoing research, continuous model evaluation, and active efforts to mitigate and eliminate biases in AI systems.
